Learning with Molecules beyond Graph Neural Networks

We demonstrate a deep learning framework which is inherently based in the highly expressive language of relational logic, enabling to, among other things, capture arbitrarily complex graph structures. We show how Graph Neural Networks and similar models can be easily covered in the framework by specifying the underlying propagation rules in the relational logic. The declarative nature of the used language then allows to easily modify and extend the propagation schemes into complex structures, such as the molecular rings which we choose for a short demonstration in this paper.

==> img/hydrogen.tex <==
\begin{tikzpicture}

\node[atom, ball color=blue!50!white, label=below left:$a(h_1)$, label=above:{$b(h_1,h_2)$}] at (0,6) (h3) {\textbf{H\textsuperscript{\tiny 1}}};
\node[atom, ball color=blue!50!white, label=above right:$a(h_2)$, label=below:{$b(h_2,h_1)$}] at (1.2,5.3) (h4) {\textbf{H\textsuperscript{\tiny 2}}};

\end{tikzpicture}

==> img/simple.tex <==
\begin{tikzpicture}
[transform shape,rotate=0, node distance=2.0cm and 2.0cm,
ar/.style={->,>=latex},
mynode/.style={
  draw, scale = 1.0,  minimum size=1cm, rounded corners,left color=white,
  minimum height=1cm,
  align=center
  }
]

\tikzstyle{recnode}  =  [mynode, right color=white!30!white]


\node[recnode, circle, label={left:{$f(x)=1$}}] (n1) {$n_1$};

\node[recnode, label={left:{$f(x)=w_1 \cdot x$}}] (n2) [above left = 1cm and 1cm of n1] {$n_2$};
\node[recnode, label={right:{$f(x)=w_1 \cdot x$}}] (n3) [above right = 1cm and 1cm of n1] {$n_3$};

\node[recnode, label={left:{$f(x,y)=w_2 \cdot x + w_2 \cdot y$}}] (n4) [above right = 1cm and 1cm of n2] {$n_4$};

\draw[->] (n1) -> node[below,sloped] {$w_1$} (n2);
\draw[->] (n1) -> node[below,sloped] {$w_1$} (n3);

\draw[->] (n3) -> node[above,sloped] {$w_2$} (n4);
\draw[->] (n2) -> node[above,sloped] {$w_2$} (n4);

\end{tikzpicture}

==> img/simple_compressed.tex <==
\begin{tikzpicture}
[transform shape,rotate=0, node distance=2.0cm and 2.0cm,
ar/.style={->,>=latex},
mynode/.style={
  draw, scale = 1.0,  minimum size=1cm, rounded corners,left color=white,
  minimum height=1cm,
  align=center
  }
]

\tikzstyle{recnode}  =  [mynode, right color=white!30!white]


\node[recnode, circle, label={left:{$f(x)=1$}}] (n1) {$n_1$};

\node[recnode, label={left:{$f(x)=2 w_1 \cdot x$}}] (n2) [above of = n1] {$n_{2-3}$};
% \node[recnode, label={right:{$f(x)=w_1 \cdot x$}}] (n3) [above right of = n1] {$n_3$};

\node[recnode, label={left:{$f(x,y)=2 w_2 \cdot x$}}] (n4) [above of = n2] {$n_4$};

\draw[->] (n1) -> node[left] {$w_1$} (n2);
% \draw[->] (n1) -> node[below,sloped] {$w_1$} (n3);

% \draw[->] (n3) -> node[above,sloped] {$w_2$} (n4);
\draw[->] (n2) -> node[left] {$w_2$} (n4);

\end{tikzpicture}

==> img/water.tex <==
\begin{tikzpicture}

\node[atom, ball color=red!50!white, label={[xshift=-0.7cm, yshift=-2.9cm]$b(o_1,h_2)$}, label={[xshift=-0.7cm, yshift=0cm]$b(o_1,h_1)$}, label=left:{$a(o_1)$}] at (0,1) (o1) {\huge \textbf{O\textsuperscript{{\tiny 1}}}};

\node[atom, circle, ball color=blue!50!white, label=above right:{$a(h_2)$}, label=below:{$b(h_2,o_1)$}] at (1,-0.1) (h1) {\textbf{H\textsuperscript{\tiny 2}}};
\node[atom, circle, ball color=blue!50!white, label=below right:{$a(h_1)$}, label=above:{$b(h_1,o_1)$}] at (1,2.1) (h2) {\textbf{H\textsuperscript{\tiny 1}}};

\end{tikzpicture}
